GamePlan: Game-Theoretic Multi-Agent Planning with Human Drivers at Intersections, Roundabouts, and Merging

We present a new method for multi-agent planning involving human drivers and autonomous vehicles (AVs) in unsignaled intersections, roundabouts, and during merging. In multi-agent planning, the main challenge is to predict the actions of other agents, especially human drivers, as their intentions are hidden from other agents. Our algorithm uses game theory to develop a new auction, called GamePlan, that directly determines the optimal action for each agent based on their driving style (which is observable via commonly available sensors). GamePlan assigns a higher priority to more aggressive or impatient drivers and a lower priority to more conservative or patient drivers; we theoretically prove that such an approach is game-theoretically optimal prevents collisions and deadlocks. We compare our approach with prior state-of-the-art auction techniques including economic auctions, time-based auctions (first-in first-out), and random bidding and show that each of these methods result in collisions among agents when taking into account driver behavior. We compare with methods based on DRL, deep learning, and game theory and present our benefits over these approaches. Finally, we show that our approach can be implemented in the real-world with human drivers.

==> Sections/1-intro_old.tex <==
\section{Introduction}
\label{sec: introduction}
\input{NeuRIPS2020/img/cover/cover}

Autonomous vehicles (AVs) have been an active area of research with advances in perception~\cite{perception_review}, prediction~\cite{chandra2019traphic}, planning and navigation~\cite{schwarting2018planning}. Such efforts have led to successful deployment of AVs in sparse traffic and highway environments. To expand this deployment to dense urban traffic, planning and navigation methods are being developed for urban scenarios consisting of intersections, frequent merging, and roundabouts. Navigation in such scenarios, however, is hard due to multiple and simultaneous interactions between AVs and human drivers which are often unpredictable. In order to model these interactions, current state-of-the-art methods in navigation and planning~\cite{schwarting2018planning} rely on implicit or explicit communication between AVs and human drivers using turn signals, flashing headlights, or right-of-way rules. However, there are many instances in everyday life when drivers are either unable to communicate with other drivers or choose to ignore such communications (\textit{e.g.,} traffic-agents in India~\cite{arrivesafe}), causing road accidents~\cite{roh2020multimodal, road_accidents1}. 
% In this paper, we formulate the problem of multi-agent planning at uncontrolled and unsignaled traffic scenarios like intersections, roundabouts, and merging~\cite{roh2020multimodal, tian2020game}. 

In addition to road accidents, the absence of communication or right-of-way rules results in collisions and deadlocks among traffic-agents~\cite{road_accidents1, arrivesafe}. For instance, consider a commonly occurring scenario consisting of four human drivers arriving at a four-way, unsignaled intersection at exactly the same time (Figure~\ref{fig: cover}). A very conservative driver may decide to play it safe and wait, choosing to go last and letting others pass the intersection first. This is the safest choice for this driver; however, one of the other three drivers with a similar conservative disposition could follow the same line of thinking. This leads to a frustrating deadlock between these two drivers (Figure~\ref{fig: cover3}). Conversely, two aggressive drivers, each deciding to take the initiative and move first at the same time, may lead to a collision (Figure~\ref{fig: cover1}). 
% Our goal is to design efficient and reliable navigation methods to handle such situations safely.
% We explore navigation in such scenarios to help agents navigate these situations successfully. 

Despite recent progress in planning and navigation in urban traffic scenarios, there is still no theoretical framework in place that formulates this problem and characterizes its solutions. Open questions in this area include deciding on optimality criteria for a successful navigation solution, determining the hardness of the problem, knowing whether a solution is always guaranteed to exist and if not, characterizing the conditions under which a solution can be guaranteed. Current planning and navigation methods in autonomous driving can perform collision-free navigation among dynamic obstacles provided that the obstacles can communicate their motion and dynamics information to other agents~\cite{schwarting2018planning}. However, these methods are unable to successfully navigate uncontrolled and unsignaled traffic scenarios in a collision- and deadlock-free manner. One of the reasons is that most of the state-of-the-art planning and navigation methods operate at the motion- and trajectory-level and do not take into account higher-level interactions between human drivers. Human drivers regularly rely on these high-level social interactions to prevent collisions and resolve deadlocks by recognizing aggressive drivers and allowing them to move first. In such scenarios, new planning algorithms must determine a turn-based ordering~\cite{carlino2013auction, sayin2018information, rey2021online, lin2021pay, vasirani2012market} that decides \textit{who} moves \textit{when}.

Game theoretic approaches, initiated by Dresner and Stone~\cite{dresner2008multiagent}, have shown that auctions, a game theoretic mechanism for allocating goods to bidders, serve as an effective framework to compute incentive compatible and welfare maximizing turn-based orderings at unsignaled intersections~\cite{carlino2013auction, sayin2018information, rey2021online}. Each agent (bidder) bids whether to move or wait. A centralized auction program collects the bids and allocates each agent a position in the turn-based ordering (goods). Auction-based multi-agent planning methods are effective; however, a major limitation is that the current auction formats rely on a monetary-based bidding system where users are required to maintain a ``wallet''~\cite{carlino2013auction}. While such bidding systems are successful in controlling congestion at intersections, they imply a strong assumption that humans are aware of the monetary values of their preferences which may not hold in real world scenarios. Consequently, such auctions have only been used in simulation. To extend auction-based planning to real-world traffic scenarios, new bidding strategies must be developed that take into account driver behavior.

% Write about CMetric here.
Recent work in trajectory analysis and driver behavior modeling~\cite{cmetric, schwarting2019social} can classify the aggressiveness and conservativeness of drivers based on the drivers' trajectories. In particular, CMetric~\cite{cmetric} models the aggressiveness of an agent by measuring the likelihood of that agent performing various aggressive maneuvers such as overspeeding, overtaking, and so on. Furthermore, these techniques are online and can predict driver behavior on real trajectory data and used for trajectory or behavior prediction.
%Recently, these behavior modeling techniques have been used to improve planning in single-agent environments~\cite{bgap}.

% While these driver behavior models have been used for single-agent planning~\cite{bgap} in simple and sparse highway environments, extending them to multi-agent planning in unsignaled and uncontrolled traffic scenarios is a promising direction.


\subsection{Main Contributions}

We present the first theoretical framework for game-theoretic multi-agent planning with human drivers and autonomous vehicles (AVs) at unsignaled intersections, roundabouts, and during merging. We formulate the multi-agent planning problem as a game-theoretically optimal sponsored search auction (SSA)~\cite{roughgarden2016twenty} that computes a turn-based ordering that is incentive compatible and welfare maximizing in polynomial time. Our turn-based ordering determines \textit{which agent} moves \textit{when} thereby preventing collision and deadlocks.

We show this problem is NP-complete and describe conditions for when a solution may exist. Furthermore, we unify current planning and navigation approaches under this framework and discuss how future solutions may be obtained using these theoretical results. Using this framework, we give a heuristic algorithm based on driver behavior that runs in polynomial time to solve the multi-agent navigation problem. Specifically, we use a novel bidding strategy using the driving behaviors~\cite{cmetric} of AVs and human drivers. 
% Specifically, we use the CMetric behavior prediction algorithm~\cite{cmetric} to compute the behavior profile of each agent from its trajectory. 
% We present a new centralized multi-agent game-theoretic planning algorithm called \textsc{GamePlan} for uncontrolled and unsignaled intersections, merging, and roundabouts with human drivers and AVs. We formulate the multi-agent planning problem as a game-theoretically optimal sponsored search auction (SSA)~\cite{roughgarden2016twenty} that computes a turn-based ordering that is incentive compatible and welfare maximizing in polynomial time. Our turn-based ordering determines \textit{which agent} moves \textit{when} thereby preventing collision and deadlocks.

% In the SSA formulation, we use a novel bidding strategy using the driving behaviors of AVs and human drivers. Specifically, we use the CMetric behavior prediction algorithm~\cite{cmetric} to compute the behavior profile of each agent from its trajectory. 
Our main contributions can be summarized as follows,

\begin{enumerate}[noitemsep]

    \item A new theoretical framework for game-theoretic multi-agent planning with human drivers and AVs at intersections, roundabouts, and during merging. We prove this problem is NP-complete and characterize heuristic and approximate solutions to this problem. 
    \item We propose a heuristic algorithm to solve his problem by integrating driver behavior modeling using trajectory analysis with sponsored search auctions. We propose a novel bidding strategy in which agents bid on whether to move or wait based on their driving behavior that is computed using CMetric~\cite{cmetric}.
    % Specifically, we show through two experiments conducted in the real world that such an auction mimics how real human drivers regularly resolve deadlock conflicts at intersections, roundabouts, and during merging.
 
   \item We show that our approach is game-theoretically optimal \textit{i.e.} it is incentive compatible, welfare maximizing, and can be computed in polynomial time, in a wide range of scenarios.
   
   \item \model~models \textit{non-ideal} agents. Non-ideal agents (human drivers or AVs) do not have access to the actions and objectives of other agents. This is in contrast to \textit{ideal} agents used in prior planning algorithms that have access to the actions and objectives of every other agent in the environment~\cite{cleac2019algames, cleac2020lucidgames, wang2020game}.
   
   \item Our approach can be extended to real world scenarios. In Section~\ref{sec: experiments_and_results} and Figure~\ref{fig: real_world}, we show two scenarios where we validate our model using human drivers in the real world.
\end{enumerate}


We evaluate our method by comparing it with state-of-the-art planning methods~\cite{roh2020multimodal, li2020game, tian2020game, liu2020decision, isele2018navigating} for unsignaled and uncontrolled environments and show a maximum reduction in the number of collisions and deadlocks by up to $30\%$. Additionally, we compare our algorithm with an ablated version that does not use turn-based orderings and show that the time taken for all agents to navigate the scenarios increases in the latter case. Finally, we demonstrate \model~in two real-world merging scenarios involving real human drivers and show that our game-theoretic model works well for real-world scenarios.
% What is Task Planning
% Autonomous vehicles (AVs) are emerging as an active area of research with advances in perception~\cite{perception_review}, prediction~\cite{chandra2019traphic}, planning, and navigation~\cite{schwarting2018planning}. \trisha{Connection missing +Re-write this sentence}
% % In particular, progress in planning and navigation research has led to deployment of AVs in sparse traffic and highway environments. 
% Encouraged by the successful deployment of AVs in sparse traffic scenarios, new planning methods are being developed for extending navigation to dense urban scenarios consisting of intersections, frequent merging, and roundabouts involving multiple simultaneous interactions between AVs and human drivers. In order to model these interactions, current state-of-the-art in navigation and planning rely on implicit or explicit communication between AVs and human drivers using turn signals, flashing headlights, or right-of-way rules. However, there are many instances in everyday life when drivers are either unable to communicate with other drivers or simply choose to ignore to do so (for \textit{e.g.} traffic-agents in India~\cite{arrivesafe}) causing road accidents~\cite{road_accidents1, roh2020multimodal}. Therefore, new methods must be developed to address the problem of decentralized planning at uncontrolled and unsignaled (non-communicative agents) intersections, roundabouts, and during merging~\cite{roh2020multimodal, tian2020game}. \trisha{last sentence needs to go in next paragraph}

% The absence of communication or right-of-way rules result in collisions and deadlocks among traffic-agents\footnote{We use the terms ``traffic-agent'' and ``agent'' interchangeably.}. To see why, consider a commonly occurring scenario consisting of four human drivers arriving at a four-way unsignaled intersection at exactly the same time. Now a very conservative driver may decide to play it safe and wait, choosing to go last and let others pass the intersection first. This is the safest choice for this driver; however, one of the other three drivers with a similar conservative disposition could follow the same line of thinking. This leads to a frustrating deadlock between these two drivers. Conversely, two aggressive drivers, each deciding to take the initiative and move first at the same time, may lead to a potential collision. 

% \trisha{State the goal of successful planning methods + then explain the issues with current methods + citations misssing }Current planning methods in autonomous driving are unable to perform collision- and deadlock-free navigation at unsignaled traffic scenarios since they plan at the motion and trajectory level and do not take into account higher-level interactions between human drivers. Human drivers regularly rely on these high-level social interactions to prevent collisions and resolve deadlocks by recognizing aggressive drivers and allowing them to move first. Therefore, new planning algorithms must implicitly determine a turn-based ordering that decides \textit{who} moves \textit{when}. Once such an ordering has been decided, each agent is allowed to move on their turn without having to conflict with other agents thereby resolving collisions and deadlocks.

% % There are certain challenges that arise with such an approach; namely, orderings must be \textit{envy-free} and acceptable to all agents and they must be \textit{truthful}. EXPLAIN TESLA. In other words, no driver should be incentivised to falsely modify the ordering so they are assigned an earlier turn. 

% \trisha{connection required} A line of research in game theory, initiated by Dresner and Stone~\cite{dresner2008multiagent}, has shown that auctions serve as an effective framework to compute envy-free and truthful turn-based orderings in unsignaled intersections~\cite{carlino2013auction, sayin2018information, rey2021online}. Each agent submits their preferences over a set of actions in the form of bids to an auction program which allocates each agent a position in the turn-based ordering. Auction-based multi-agent planning methods are effective; however, a major limitation is that the current auction formats rely on a monetary-based bidding system where users are required to maintain a ``wallet''~\cite{carlino2013auction}. While such bidding formats are successful in controlling congestion at intersections, they imply a strong assumption that humans are aware of the monetary values of their preferences, which is realistically not the case, prohibiting their application in the real world. In this regard, such auctions have only been used in simulation.

% {No connection to this paragraph at all}
% In the robotics literature, it has been recently shown that a traffic-agents preference over actions at intersections, roundabouts, and during merging are determined by the driving behavior of the agent. Specifically, the more aggressive an agent is, the more likely they will move first during intersections or roundabouts and cut off other drivers during merging. 
% % While the method by Wang et al.~\cite{wang2020game} introduces a risk-aware navigation model for simulated agents, they do not model real human behavior. 
% One of the goals of this paper is to combine these ideas from game theory and robotics to propose a new auction format that replaces the current monetary-based bidding system with a behavior-based one. 

% \subsection{Main Contributions}
% \label{subsec: main_contributions}

% We propose a new decentralized game-theoretic planning algorithm, called \textsc{GamePlan}, for intersections, merging, and roundabouts involving non-communicating human drivers and AVs. We frame the multi-agent planning problem as a sponsored search auction~\cite{roughgarden2016twenty} that determines an ordering in which agents shall move based on the risk-sensitivity of the human driver. We use an online behavior prediction model that can infer the aggressiveness (risk-seeking) and conservativeness (risk-averse) behavior of a human driver based solely on the trajectory of their vehicle. The main advantages of \model~are:

% \begin{itemize}
%     \item \textit{Optimality and efficiency guarantees:} We show that the orderings computed using \model~are truthful, envy-free, and acceptable to all agents. Further, we show that such orderings can be computed in polynomial time.
    
%     \item \textit{Real world application:} We show that \model~can be applied in real world environments.
    
%     \item \textit{Integration with motion planners:} \model~is complementary to existing research in trajectory and motion planning. Specifically, \model~may be used initially to establish a  turn-based ordering for traffic-agents followed by using trajectory and motion planners that can plan safe paths for the agent at the current turn.
    
%     \item \textit{Preventing collisions and deadlocks:} We show that \model~reduces the collision frequency in four-way intersection scenarios by up to $30\%$ and improves deadlock resolution by up to $20\%$ compared to when agents use planning methods without a turn-based ordering mechanism.
% \end{itemize}


% Through our experiments, we first show that having such an auction reduces the collision frequency in four-way intersection scenarios by up to $30\%$, compared to when agents use a trajectory planner but do not leverage any form of task planning. We then demonstrate \model~in a real world merging scenario with two human drivers. 

% A recent study~\cite{road_accidents1} on the causes of road accidents in India reports that $78\%$ of total accidents occur due to human drivers not adhering to general traffic rules. Therefore, if autonomous driving is to become a reality across the world, then new approaches for task planning for AVs cannot assume perfect communication with human drivers.
% While the recent advances in autonomous driving have contributed to the deployment of AVs in sparse traffic and highway environments, it remains a challenge for AVs to navigate in dense urban environments. It has been shown~\cite{bgap, cleac2019algames, cleac2020lucidgames, wang2020game} that in order to navigate among human drivers, AVs must be able to plan ahead taking into consideration the actions of the human drivers which can, however, often be unpredictable. In robotics, a lot of work has gone into developing robust and accurate planning methods~\cite{schwarting2018planning} that plan for an ego-vehicle in single-agent environments. In this work, we consider planning in multi-agent traffic environments where the goal is to predict the high level symbolic actions for every agent at the task level (``accelerate'', ``brake'', ``turn left/right'', etc.). 


% There are different types of planning in autonomous driving including motion planning, trajectory planning, and task planning. The first two categories of planning are In this paper, we tackle task planning in multi-agent traffic scenarios. A crucial problem problems in autonomous driving is task planning, in which the goal is to predict the high level symbolic actions for the AV at the task level (``accelerate'', ``brake'', ``turn left/right'', etc.). 

% Task planning is difficult in multi-agent scenarios involving both human drivers and AVs such as intersections, merging, roundabouts and so on, due to the need to integrate social interactions between road-agents with task planning~\cite{bgap, schwarting2019social}.
% For example, suppose an AV must turn left at a four-way intersection with human drivers. The AV first has to decide whether it is its turn to move based on right-of-way, before planning the left turn.
% It is important to note that task planning is different from motion planning, in that motion planning answers the question, \textit{``How do I get there?''}, while task planning aims to answer an even more fundamental question, \textit{``What path do I take?''.}

% WHat is the problem in TP we are solving
% Most existing task planning frameworks~\cite{tp1, tp2} assume some form of communication between AVs and human drivers using turn signals, flashing headlights, or even relying on right-of-way. However, in many parts of the world (\textit{e.g.} India) human drivers do not obey turn signals or right-of-way, increasing the likelihood of road accidents. A recent study~\cite{road_accidents1} on the causes of road accidents in India reports that $78\%$ of total accidents occur due to human drivers not adhering to general traffic rules. Therefore, if autonomous driving is to become a reality across the world, then new approaches for task planning for AVs cannot assume perfect communication with human drivers.


% The main challenge with task planning in multi-agent traffic scenarios without communication is to predict the optimal actions of human drivers. Such actions are typically guided by human incentives which are unknown to the other agents. For instance, consider a scenario where an AV is trying to merge onto a highway with a human driver in the target lane. An aggressive human driver will accelerate and not allow the AV to merge whereas a conservative human driver will slow down to allow the AV to merge onto the highway. 


% In the example above, both the aggressive and conservative human driver, along with the AV, will submit action preferences to the auction program. The aggressive driver, having submitted a higher preference to accelerate will be given priority to act first over the AV whereas in the second case, the preference of the AV to act first is stronger than that of the conservative human driver, thus allowing the AV to merge onto the highway.

% Such auction mechanisms have mostly been used in intersection scenarios


% Current research efforts have begun to use game theory to model such incentive-based decision making among intelligent agents.
% Game theory has been used to model interactions between human drivers in multi-agent traffic environments to predict future actions.
% In a game-theoretic sense, it can be assumed that each agent strives to act in their best interest. The second challenge, which remains unsolved to the best of our knowledge, is to predict the \textit{optimal} action of each agent from the action set (depending on the inferred driver behavior) in a multi-agent scenario involving human drivers and AVs. 
% However, the state-of-the-art in game-theoretic methods for planning~\cite{gt1, gt2}, navigation~\cite{wang2020game, cleac2019algames, cleac2020lucidgames}, and behavior modeling~\cite{schwarting2019social} assume that every agent knows the objective function of all other agents, which is unrealistic in the real world. To reduce the dependence on this assumption, follow-up works~\cite{gt2, cleac2020lucidgames, cleac2019algames} have explored inverse optimal control or IOC (also known as inverse reinforcement learning in some literature) to learn the agents' objective functions from given data. However, IOC-based methods do not provide theoretical guarantees of an optimal solution, are susceptible to poor generalization~\cite{gt2}, and require expensive computations~\cite{rabinowitz2018machine}. 
% Without knowledge of the behavior of the driver, it is impossible to know which of the two scenarios is more likely. The first step in task planning without communication, thus, is for a central controller to be able to infer human driver behavior in an online manner. Some approaches~\cite{cmetric, schwarting2019social} have been proposed recently that infer the aggressiveness and conservativeness of human drivers.

% The second challenge is to select the \textit{optimal} action of each agent, which depends on the incentives or objectives of each agent. However, human drivers generally do not know the objectives, incentives, or actions of other drivers. Game theory has been used to model interactions between human drivers in multi-agent traffic environments to predict future actions.
% In a game-theoretic sense, it can be assumed that each agent strives to act in their best interest. The second challenge, which remains unsolved to the best of our knowledge, is to predict the \textit{optimal} action of each agent from the action set (depending on the inferred driver behavior) in a multi-agent scenario involving human drivers and AVs. 
% However, the current state-of-the-art in game-theoretic methods for planning~\cite{gt1, gt2}, navigation~\cite{wang2020game, cleac2019algames, cleac2020lucidgames}, and behavior modeling~\cite{schwarting2019social} assume that every agent knows the objective function of all other agents, which is unrealistic in the real world. To reduce the dependence on this assumption, follow-up works~\cite{gt2, cleac2020lucidgames, cleac2019algames} have explored inverse optimal control or IOC (also known as inverse reinforcement learning in some literature) to learn the agents' objective functions from given data. However, IOC-based methods do not provide theoretical guarantees of an optimal solution, are susceptible to poor generalization~\cite{gt2}, and require expensive computations~\cite{rabinowitz2018machine}. 

% The second step in task planning without communication, therefore, is to predict the optimal action for each agent in a scenario involving human and AVs with completeness guarantees in a computational tractable manner.


% The only assumption in our framework is that we know the positions of the human drivers, which can be easily obtained using sensors such as depth cameras, stereo cameras, radars, or lidars. Using our framework, we propose two task planning algorithms with completeness guarantees that differ based on their strategies for modeling human driver behavior. Our main contributions include:

% \begin{enumerate}
%     \item \model, a novel game-theoretic task planning framework for various multi-agent traffic scenarios where agents may not communicate with each other. The main advantages of \model~are that resulting task planning algorithms are complete, computationally tractable, and effective.
% \end{enumerate}

% We validate \model~through experiments performed in the real world with human drivers as well as in simulation. We show that by using \model, we can reduce collisions in a four-way intersection by $30\%$.
% As human drivers, we are able to infer the behaviors of other human drivers~\cite{quartz-article, cuzzolin2020knowing, theoryofmind}, without explicit communication, simply by observing the motion of their vehicles. As an example, if a vehicle is weaving through traffic, other drivers typically infer that the driver of the weaving vehicle is aggressive, and accordingly keep their distance from that vehicle.



% Indeed, road safety organizations assert that a general lack of respect for traffic rules in India is a contributing factor for road collisions~\cite{arrivesafe} with over
% $78\%$ of total road accidents occurring due to the human driver not adhering to the traffic rules~\cite{road_accidents1}.


% As of today, current state-of-the-art motion planning solutions for autonomous driving answer the latter question by either assuming a starting position and a goal position, or by sampling the entire space of start-end position configurations. Neither approach is suitable, however, when it comes to highly uncertain environments consisting of human drivers. Human drivers act in unpredictable and irrational ways necessitating AVs to incorporate higher order planning at the task level. For instance, in the earlier example, assume there is rush hour traffic along the highway, then the AV may need to additionally plan a task to start switching over to the exit lane earlier than the programmed time so as not to miss the exit. Such an example of higher-order planning cannot be achieved by SOTA motion planning, rather through task planning.

% Prior Methods for task Planning


==> Sections/5-decision.tex <==
\section{Validating the Behavior Model}
\label{sec: validating_cetric}

A major assumption made by our approach is the availability of a reliable driver behavior prediction model. We use the CMetric algorithm for behavior prediction introduced by Chandra et al.~\cite{cmetric} with a variant being used in~\cite{chandra2019graphrqi}. Although validating the CMetric algorithm is not a focus of this paper, we summarize some of the validation and evaluation results from these prior works.

In~\cite{cmetric}, the authors introduce a new metric to validate the CMetric algorithm called the Time Deviation Error (TDE). The TDE measures the temporal difference between the time-stamps when a human identifies an aggressive behavior and when that same behavior is modeled using CMetric. For example, if a vehicle executes a rash overtake at the $8^\textrm{th}$ video frame and CMetric predicts the behavior at the $10^\textrm{th}$ frame, then the TDE$=0.1$ seconds, assuming $20$ frames per second. A lower value for TDE indicates a more accurate behavior prediction model. CMetric has an average TDE of less than $1$ second. In~\cite{chandra2019graphrqi}, the authors combine CMetric with machine learning and use classification accuracy as an evaluation metric. This metric is simply measured as the  fraction of correctly predicted behaviors, weighted by class frequencies. CMetric achieves a weighted classification accuracy of up to $90\%$. We refer the reader to the original papers on CMetric for further details regarding the experimentation.






==> Sections/back.tex <==
\section{Background and Problem Formulation}
In this section, we begin by defining several key terms and stating the problem statement followed by the assumptions made in our approach. We briefly summarize the CMetric algorithm~\cite{cmetric} for behavior modeling and prediction and provide an overview on sponsored search auctions~\cite{roughgarden2016twenty}, which are widely used in game theory.

\subsection{Problem formulation}
\label{subsec: problem_formulation}

We frame navigating unsignaled intersections, roundabouts, and merging scenarios as a multi-agent game-theoretic non-sequential decision-making problem. We consider three unsignaled and uncontrolled traffic scenarios or environments -- intersections, merging, and roundabouts with multiple non-communicating human drivers and AVs. In each of the three scenarios, we refer to a traffic-agent as ``active'' if they participate in the decision-making process for navigating the scenario. For example, the lead traffic-agents in each service lane of a four-way intersection are active vehicles, while agents waiting in line behind their respective lead vehicle are non-active agents. We denote the active agents as a set $\mathcal{A} = \{a_1, a_2, \ldots a_n \}$. The action space for each active agent is a discrete set consisting of finite acceleration values. The state space consists of the position $x_t \in \mathcal{X}$ and velocity $v_t$ of each agent measured in a global coordinate frame (\textit{e.g.} GPS coordinates or $3-$D points obtained using GPS and lidars, respectively).

\subsection{Modeling human driver behavior}
\label{subsec: cmetric_background}

Each active agent is characterized by a behavior profile, $\bm{\zeta}_i$, which can be obtained via recent behavior modeling algorithms such as the SVO~\cite{schwarting2019social} and CMetric~\cite{cmetric}. In this work, we use CMetric to quantify the aggressiveness or conservativeness of a traffic-agent. This model provides an objective measure of aggressiveness based on driving maneuvers such as overspeeding, overtaking and so on. We briefly summarize the CMetric algorithm. To determine if an agent is aggressive or conservative, the algorithm begins by reading the trajectories of the ego-agent and surrounding vehicles via cameras or lidars during any time-period $\Delta t$. The trajectory of an agent is represented by 

\[\Xi_{\Delta t} = \{x_t \ | \ t = t_0, t_1, \ldots, t_0 + \Delta t \}.\]

\noindent In CMetric, these trajectories are represented via weighted undirected graphs $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ in which the vertices denote the positions for each agent and the edges correspond to the distances between agents. The algorithm proceeds by using these graphs to model the likelihood and intensity of driving behavior indicators like overspeeding, overtaking, sudden ``zig-zagging'' and lane-changes via centrality functions~\cite{rodrigues2019network} represented by $\Phi: \mathcal{G}\rightarrow \mathbb{R}$. These behavior indicators determine whether an agent is aggressive or conservative~\cite{sagberg2015review}. The behavior profile for $a_i$ is denoted by $\bm{\zeta}_i$ and can be computed using,

\begin{equation}
    \bm{\zeta}_i(\Xi_{\Delta t}) = \Phi(\mathcal{G}),
    \label{eq: cmetric}
\end{equation}

\noindent where $\mathcal{G}(\mathcal{V}, \mathcal{E})$ is constructed using $\Xi_{\Delta t}$. In this work, we use CMetric to compute the behavior profiles of traffic-agents, represented by a $n-$dimensional vector $\bm{\zeta},$ that is provided to the auction program.

\subsection{Assumptions}
\label{subsec: assumptions}

We assume agents (AVs and human drivers) are rational and strive to maximize their own utility which can be independent of other agents. Further, agents are \textit{non-ideal} (in contrast to ideal agents in~\cite{cleac2020lucidgames, cleac2019algames, wang2020game}) in that they do not have access to the actions, objectives, or utility functions of other agents. We make no assumptions on the motion or dynamics of traffic-agents. The state-space is fully observable by all agents (active and non-active). We assume the availability of a behavior modeling and prediction algorithm such as CMetric~\cite{cmetric} that models driving behavior as being either aggressive or conservative. This information is provided to an auction program. We assume that agents navigate through the environment one at a time and do not use traffic signals, employ right-of-way rules, or communicate with other agents.

\subsection{Sponsored search auctions (SSAs)}
\label{subsec: SSA_background}
Sponsored search auctions (SSAs) are a game-theoretic mechanism that are used extensively in internet search engines for the purpose of internet advertising~\cite{roughgarden2016twenty}. In an SSA, there are $K$ items to be allocated among $n$ agents. Each agent $a_i$ has a private valuation $\bm{v}_i$ and submits a bid $\bm{b}_i$ to receive at most one item of value $\bm{\alpha}_i$. A strategy is defined as an $n$ dimensional vector, $\bm{b} = (\bm{b}_i \cup \bm{b}_{-i})$, representing the bids made by every agent. $\bm{b}_{-i})$ denotes the bids made by all agents except $a_i$. Furthermore, let $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ and $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$. The allocation rule is that the agent with the $i^\textrm{th}$ highest bid is allocated the $i^\textrm{th}$ most valuable item, $\bm{\alpha}_i$. The utility $\bm{u}_i$~\cite{roughgarden2016twenty} incurred by $a_i$ is given as follows,

\begin{equation}
 \bm{u}_i (\bm{b}_i) =  \bm{v}_i \bm{\alpha}_i - \sum_{j=i}^k \bm{b}_{j+1} \left( \bm{\alpha}_j - \bm{\alpha}_{j+1} \right).
 \label{eq: utility_template}
\end{equation}

\noindent In the equation above, the quantity on the left represents the total utility for $a_i$ which is equal to value of the allocated goods $\bm{\alpha}_i$ minus a payment term. The first term on the right is the value of the item obtained by $a_i$. The second term on the right is the payment made by $a_i$ as a function of bids $\bm{b}_{j > i}$ and their allocated item values $\bm{\alpha}_j$. We refer the reader to Chapter $3$ in~\cite{roughgarden2016twenty} for a derivation and detailed analysis of Equation~\ref{eq: utility_template}.

In our approach, we re-cast Equation~\ref{eq: utility_template} through the lens of a human driver. More specifically, the term $\bm{v}_i \bm{\alpha}_i$ denotes the time reward gained by driver $a_i$ by moving on her turn. The payment term represents a notion of risk~\cite{wang2020game} associated with moving on that turn. It follows that an allocation of a conservative agent to a later turn (smaller $\bm{\alpha}$) also presents the lowest risk and vice-versa.

\subsection{Problem statement}

To prevent collisions and deadlocks, it is necessary to determine the order in which agents take turns to navigate the traffic scenario~\cite{carlino2013auction, dresner2008multiagent, lin2021pay, sayin2018information, schepperle2007agent, vasirani2012market}. Thus, the goal of this paper (formalized shortly via Problem~\ref{problem: prob}) is to compute an optimal turn-based ordering which is defined as follows,

% \input{NeuRIPS2020/img/overview/overview}

\begin{definition}
\textbf{Turn-based Orderings ($\bm{\sigma}$): } A turn-based ordering is a permutation $\bm{\sigma}: \mathcal{A} \rightarrow [1,n]$ over the set $\mathcal{A}$. For any $i,j \in [1,n]$, $\bm{\sigma}(a_i) = j$, equivalently $\bm{\sigma}_i = j$, indicates that $a_i$ with driving behavior $\bm{\zeta}_i$ will move on the $j^\textrm{th}$ turn.
\label{def: turn_based_ordering}
\end{definition}


\noindent There may be multiple turn-based orderings that may apply in a given scenario. However, many of them could be sub-optimal and may result in collisions and deadlocks. An optimal turn-based ordering prevents collisions and resolves deadlock conflicts.

\begin{definition}
\textbf{Optimal Turn-based Ordering ($\bm{\sigma}_{\textsc{opt}}$): } A turn-based ordering, $\bm{\sigma}$, over a given set $\mathcal{A}$ is game-theoretically optimal if it is incentive compatible, welfare maximizing, and can be computed in polynomial time\footnote{These terms are defined in Section~\ref{subsec: optimality}}.
\label{def: optimal_turn_based_ordering}
\end{definition}

\noindent We now ready to formally state our goal in this paper as follows,

\begin{problem}
In a traffic scenario (which could be an intersection, roundabout, or merging) with $n$ active road-agents, given the behavior profile $\bm{\zeta}_i$ of each agent, the goal is to compute the optimal turn-based ordering $\bm{\sigma}_\textsc{opt}  = \bm{\sigma}_1\bm{\sigma}_2\ldots\bm{\sigma}_n$.
\label{problem: prob}
\end{problem}


% \input{NeuRIPS2020/img/overview/overview}
% In game theory, a strategy is defined as an $n$ dimensional vector, $b = (\bm{b}_i \cup \bm{b}_{-i})$, representing the bids made by every agent. The goal of any optimal auction is to generate maximum welfare upon truthful bidding so that that no agent is incentivised to ``cheat'' \textit{i.e.} incentive compatible. In other words, auctions are incentive compatible when the dominant strategy for each agent is to bid their true valuation $v_i$.
% In our proposed approach, we combine the SSA with the CMetric behavior modeling algorithm to generate an auction with a novel bidding strategy. We discuss this approach in detail in the following section. 
% We conclude current section with the some standard, but important, definitions related to game-theoretic optimality.

% \begin{definition}
% \textbf{Dominant Strategy:} Bidding $\bm{b}_i$ is a dominant strategy for $a_i$ if $\bm{u}_i(\bm{b}_i, \bar \bm{b}_{-i}) > \bm{u}_i(\bar \bm{b}_i, \bar \bm{b}_{-i})$ for all $\bar \bm{b}_i \neq \bm{b}_i$.
% \end{definition}

% We now state two important definitions that are used as the basis of an optimal SSA.

% \begin{definition}
% \textbf{Incentive Compatibility:} An auction is said to be incentive compatible if for each agent, bidding $\bm{b}_i = v_i$ is a dominant strategy.
% \label{def: incentive_compatibility}
% \end{definition}

% \begin{definition}
% \textbf{Welfare Maximization:} Social welfare of an auction outcome is defined as $\sum_i v_i \bm{u}_i(\bm{b}_i)$. Welfare maximization is the task of finding the strategy $b$ that maximizes $\sum_i v_i \bm{u}_i(\bm{b}_i)$.
% \label{def: social_welfare}
% \end{definition}

% Finally, SSAs have polynomial time complexity since sorting is polynomial time~\cite{clrs}.
% \subsubsection{Sponsored Search Auctions}

% \subsubsection{Optimality and Efficiency of SSAs}




==> Tables/benefits.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Benefits of \model~over prior work in planning.}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}

\toprule
%  &  &  & \multicolumn{2}{c}{Our CMetric Measures}\\

% \cline{4-5}
Problem Setting & Approach & Methods & Assumptions/Limitations & Benefits\\
\midrule
\multirow{2}{*}{Single-agent planning with dynamic obstacles} & Geometric Methods  && \\
                                             & Learning-based Methods && \\


\multirow{2}{*}{Multi-agent planning} & Game theory  && \\
                                             & Auctions && \\
 
\bottomrule
\end{tabular}
}
\label{tab: benefits}

\end{table*}

==> Tables/notation.tex <==
\begin{table}[t]
  \caption{Symbols and notations used in this paper.}
  \label{tab: notation}
  \centering
  \resizebox{.7\columnwidth}{!}{%
  \begin{wraptable}{r}{5.5cm}
  \begin{tabular}{cl}
  \toprule
    Symbol  & Description \\
    \midrule
    $n$ & Number of traffic-agents.\\
    $a_i$ & $i^\textrm{th}$ active agent.\\
    $\mathcal{A}$ & Set of active agents. \\
    $\zeta$ & CMetric-based behavior profile (Section~\ref{subsec: cmetric_background}). \\
    $\sigma$ & Turn-based ordering (Definition~\ref{def: turn_based_ordering}). \\
    $\sigma_{\textsc{opt}}$ & Optimal turn-based ordering (Definition~\ref{def: optimal_turn_based_ordering}). \\
    $b_i$ & Bid of the $i^\textrm{th}$ active agent.\\
    $b_{-i}$ & Bid of every agent except the $i^\textrm{th}$.\\
    $v_i$ & Private valuation of the $i^\textrm{th}$ active agent.\\
    $u_i(\cdot)$ & Utility of the $i^\textrm{th}$ active agent.\\
    $t_i$ & Time taken by the $i^\textrm{th}$ active agent \\
    & to navigate the traffic scenario.\\

    \bottomrule
  \end{tabular}
  \end{wraptable} 
  }
%   }
  \vspace{-15pt}
\end{table}


==> Tables/parameters.tex <==
\begin{table}[h]
\caption{IDM and MOBIL parameters used for Conservative and Aggressive vehicle classes}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clcc} 
\toprule
Model & Parameter \Tstrut & Conservative \Bstrut &   Aggressive \\
\hline
\multirow{4}{*}{IDM}& Time gap ( $T$) \Tstrut & 1.5s      & 1.2s \\
 &Min distance ($s_0$) & 5.0 $m$ & 2.5 $m$ \\
&Max comfort acc. ($a$)     & 3.0 $m/s^2$ & 6.0 $m/s^2$\\
&Max comfort dec. ($b$) & 6.0 $m/s^2$               &  9.0 $m/s^2$ \\
\midrule
\multirow{3}{*}{MOBIL}& Politeness ($p$) & 0.5     & 0\\
& Min acc gain ($\Delta a_{th}$) & 0.2 $m/s^2$ & 0 $m/s^2$ \\
& Safe acc limit ($b_{safe}$) & 3.0 $m/s^2$ & 9.0 $m/s^2$\\
\bottomrule
\end{tabular}
}
\label{tab: parameters}
\vspace{-10pt}
\end{table}


==> table.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Main Results:} We report the Average Displacement Error (ADE) and Final Displacement Error (FDE) for prior road-agent trajectory prediction methods in meters(m). Lower scores are better and \textbf{bold} indicates the SOTA. \textbf{Revisions:} Green colored cells indicate revised results for \textit{our} method while blue colored cells indicates revised results for the original implementations \textit{GRIP} and Social-GAN method.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule[1.1pt]
\multirow{2}{*}{Dataset \newline (Pred. Len.)}                       &
\multicolumn{2}{c}{CS-LSTM }         &
\multicolumn{2}{c}{TraPHic  }         &
\multicolumn{2}{c}{Social-GAN  }         &
\multicolumn{2}{c}{GRIP  }         &
\multicolumn{2}{c}{Ours (Stream 1 only)  }  &
\multicolumn{2}{c}{Ours (Both Streams)  }            \\
&
ADE & FDE &
ADE & FDE &
ADE & FDE &
ADE & FDE &
ADE & FDE &
ADE & FDE \\
\midrule
% \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}z
Lyft (5 sec.)           &   4.423  &  8.640  & 5.031  &  9.882   &  \cellcolor{blue!20}7.860  &  \cellcolor{blue!20}14.340  & \cellcolor{blue!20}-  &  \cellcolor{blue!20}- & \cellcolor{green!20}2.23  &  \cellcolor{green!20}2.35  &  \cellcolor{green!20}\textbf{2.22} &  \cellcolor{green!20}\cellcolor{green!20}\textbf{2.33}\\ 
Argoverse (5 sec.)      &    1.050  &  3.085  & 1.039  &  3.079   &  \cellcolor{blue!20}3.610   &  \cellcolor{blue!20}5.390  & \cellcolor{blue!20}-  &\cellcolor{blue!20}- &  \cellcolor{green!20}2.06 &  \cellcolor{green!20}2.08  &  \cellcolor{green!20}\textbf{0.97} &  \cellcolor{green!20}\textbf{2.07} \\ 
Apolloscape (3 sec.)    &    2.144  &  11.699  & 1.283  &  11.674  & \cellcolor{blue!20} 3.980  & \cellcolor{blue!20} 6.750  & \cellcolor{blue!20}\textbf{1.25} &  \cellcolor{blue!20}2.34  & \cellcolor{green!20} 1.52  & \cellcolor{green!20} 1.56  &  \cellcolor{green!20}1.51 &  \cellcolor{green!20}\textbf{1.55}\\ 
NGSIM (5 sec.)  &   7.250&10.050  & 5.630&9.910  & \cellcolor{blue!20} 5.650&\cellcolor{blue!20}10.290  & \cellcolor{blue!20}1.61  &  \cellcolor{blue!20}3.16  &  \cellcolor{green!20}1.15  &  \cellcolor{green!20}1.17  &\cellcolor{green!20}\textbf{0.99}  & \cellcolor{green!20} \textbf{1.02}\\ 
\bottomrule[1.1pt]
\end{tabular}
}
\label{tab: accuracy}
% \vspace{-15pt}
\end{table}



